Exploring How Non-Prehensile Manipulation Expands Capability in Robots Experiencing Multi-Joint Failure

This work explores non-prehensile manipulation (NPM) and whole-body interaction as strategies for enabling robotic manipulators to conduct manipulation tasks despite experiencing locked multi-joint (LMJ) failures. LMJs are critical system faults where two or more joints become inoperable; they impose constraints on the robot's configuration and control spaces, consequently limiting the capability and reach of a prehensile-only approach. This approach involves three components: i) modeling the failure-constrained workspace of the robot, ii) generating a kinodynamic map of NPM actions within this workspace, and iii) a manipulation action planner that uses a sim-in-the-loop approach to select the best actions to take from the kinodynamic map. The experimental evaluation shows that our approach can increase the failure-constrained reachable area in LMJ cases by 79%. Further, it demonstrates the ability to complete real-world manipulation with up to 88.9% success when the end-effector is unusable and up to 100% success when it is usable.

==> algos/greedy-action.tex <==
\begin{algorithm}\footnotesize

\caption{Greedy Action Selection}\label{algo:greedy-asm}
\color{dusty_blue}
\KwIn{$\mathcal{E}$, a set of edges; $E$ environment state}
%$\mathcal{C}^c$, Failure-Constrained Configuration Space;
\KwOut{$\mathcal{A}$, Chosen Action}
$\mathcal{A} \longleftarrow \emptyset$\\
% \While{\textbf{not} \textsc{ObjectInGoalRegion}($E$)}{

$\mathcal{E}_T \longleftarrow \emptyset$ \tcp{Edges Scored}\\
$scores \longleftarrow \emptyset$ \\
$\mathcal{E}_s \longleftarrow \textsc{UniformlySampleSubset}(\mathcal{E})$ \\
$E_{sim} \longleftarrow E $ \tcp{set sim env}\\ 
\For{$\mathbf{e}$ in \textsc{SampleWithoutReplacement}($\mathcal{E}_s$)} {
    \textsc{SimulateRobotWithEdge($\mathbf{e}, E_{sim}$)} \\
    \If{\textsc{TargetMovedTowardsGoal}($E_{sim}$)}{
    $scores \longleftarrow scores \cup \textsc{ScoreExecution}(E_{sim}$)}\\
$\mathcal{E}_T \longleftarrow \mathcal{E}_T \cup \mathbf{e} $ \\


$E_{sim} \longleftarrow E$ \tcp{reset sim env}
}
 
$\mathcal{A}\longleftarrow \textsc{SelectBestEdge}(\mathcal{E}_T, scores, m)$\\
% $ \longleftarrow e_{best}$ \\
% }
\Return{$\mathcal{A}$}

\end{algorithm}

==> algos/intersect-edges.tex <==
% FindIntersectingEdgesAndSetTheirScore

\begin{algorithm}\footnotesize

\caption{FindIntersectingEdgesAndSet- \\ TheirScore}\label{algo:edges-score-inters}

\KwIn{$\mathcal{E}$, a set of edges, $\mathcal{S}$ the state of the environment}
\KwOut{$\mathcal{E}_I$, a set of edges that intersect with the object}
$\mathcal{E}_I \longleftarrow \emptyset$\\
\For{$edge$ in $\mathcal{E}$} {
\textsc{SimulateRobotWithEdge($edge$, $\mathcal{S}$)} \\
\If{\textsc{TargetObjectMoved($\mathcal{S}$)}}{
$d \longleftarrow$ \textsc{GetObjectDistanceToGoal($\mathcal{S}$)}\\
$edge\cdot score \longleftarrow \frac{1}{d}$ \\
$\mathcal{E}_I \longleftarrow \mathcal{E}_I \cup edge $
}

\textsc{ResetSimEnvironment()}
}

\Return{$\mathcal{E}_I$}
\end{algorithm}

% $E_n \longleftarrow$

==> algos/kino-map.tex <==
\begin{algorithm}\footnotesize

\caption{Kartographer}\label{algo:kino-map}

\KwIn{$\mathcal{R}$, the state of the robot; $discr$, discretizationSize}
\KwOut{$\mathcal{E}$, a set of edges approximating $\mathcal{F}$}

$\mathcal{E} \longleftarrow \emptyset$ \\
$q_{limits} \longleftarrow$  \textsc{getJointAnglesLimits}$(\mathcal{R})$  \\
$qs \longleftarrow$ \textsc{DiscretizeJointSpace($q_{limits}, discr$)} \\
\For{$q$ in $qs$}{
$ee_{pos} \longleftarrow$ \textsc{ForwardKinematics}$(q)$ \\
\If{\textsc{IsInWorkspaceLimits($ee_{pos}$)}}{
$e \longleftarrow Edge()$ \\
$e\cdot q_{init} \longleftarrow q$ \\
$stepSize \longleftarrow$ \textsc{SampleStepSize()} \\
$e\cdot q_{final} \longleftarrow q_{init}.Interpolate(stepSize)$ \\
$e\cdot qdot \longleftarrow$ \textsc{SamplePrimitiveVelocity()} \\
$\mathcal{E} \longleftarrow \mathcal{E} \cup e$
}
}


\Return{$\mathcal{E}$}

\end{algorithm}

% To generate
% the failure case edges for the robot, we first identify the
% new reachable volume of the robot in joint space, as shown
% in Figure 2. For the remaining useable joints, we identify
% principal motion joints that impart the most significant in-
% teraction point motion and make a dense grid of joint con-
% figurations between the lowest and highest ranges relevant
% to the environment. We apply dynamic motions to these
% principal motion joints, which provide the most movement
% and force in a specific direction and save their trajectories
% as edges.

==> algos/lazy-action.tex <==
\begin{algorithm}\footnotesize

\caption{Lazy Action Selection}\label{algo:lazy-asm}
\color{dusty_green}
\KwIn{$\mathcal{E}$, a set of edges; $E$ environment state}
\KwOut{$\mathcal{A}$, Chosen Action}
$E_{sim} \longleftarrow E $ \tcp{set sim env}\\ 
\For{$\mathbf{e}$ in \textsc{SampleWithoutReplacement}($\mathcal{E}_s$)} {
    \textsc{SimulateRobotWithEdge($\mathbf{e}, E_{sim}$)} \\
    \If{\textsc{TargetMovedTowardsGoal}($E_{sim}$)}{
    $\mathcal{A} \longleftarrow \mathbf{e}$\\
    \textbf{break}
    }
$E_{sim} \longleftarrow E$ \tcp{reset sim env}
}
\Return{$\mathcal{A}$}

\end{algorithm}

==> algos/pick-actions.tex <==
\begin{algorithm}\footnotesize

\caption{Pick Actions.}\label{algo:pick-actions}

\KwIn{$n$, number of samples; $e$, edges; $o$, movable objects;\\$b_{RA}$, random action bias; $b_{IA}$, indirect action bias}
\KwOut{$\mathcal{A}$, chosen actions}

$\mathcal{I}, \mathcal{O} \longleftarrow$ \textsc{FindIntersectingEdges}($e$, $o$)\\

$objects \longleftarrow \emptyset$\\
$ee \longleftarrow \emptyset$\\
$\mathcal{I}_{target}, \mathcal{O}_{target} \longleftarrow$ \textsc{FindTarget}($e$, $o$)\\
\If{$rand() > b_{IA}$} {
    $ee \longleftarrow ee \cup I_{target}$
}
\Else {
    $ee \longleftarrow ee \cup (I \cap I_{target})$
}

$\mathcal{A} \longleftarrow \emptyset$ \\
$n_{rand} = b_{RA} * n$

\For{i = 1 \ldots n} {
    \For{j = 1 \ldots $n_{rand}$} {
        $\mathcal{A} \longleftarrow \mathcal{A} \; \cup$ \textsc{PickRandom}($e$)\\
    }
    $sorted\_e \longleftarrow$ \textsc{PriorityQueue}($e$)\\
    \For{j = 1 \ldots $n - n\_rand$} {
        $a \longleftarrow$ \textsc{POP}($sorted\_e$)\\
        \If{$a \notin \mathcal{A}$}{
            $\mathcal{A} \longleftarrow \mathcal{A} \cup a$
        }
    }
}

\Return{$\mathcal{A}$}

\end{algorithm}

==> algos/random-action.tex <==
\begin{algorithm}\footnotesize

\caption{Random Action Selection}\label{algo:random-asm}
\color{dusty_pink}
\KwIn{$\mathcal{E}$, a set of edges; $E$ environment state}
%$\mathcal{C}^c$, Failure-Constrained Configuration Space;
\KwOut{$\mathcal{A}$, Chosen Action}

$e \longleftarrow \textsc{RandomUniformSelect}(\mathcal{E})$\\
$\mathcal{A} \longleftarrow e$ \\
\Return{$\mathcal{A}$}

\end{algorithm}

==> definitions/control-mechanism.tex <==
\begin{definition}[Control Mechanism]\label{def:control-mechanism}
Given a vector of control parameters $u \in \mathcal{U}_{MP}$ from a set of feasible parameters corresponding to a motion primitive $MP$, the \textsl{control mechanism} $\phi_{MP}$ generates a robot trajectory that executes $u$.
\begin{center}
$\phi_{MP} \longrightarrow \tau: [0, 1]$ s.t. $\tau(0) = q_s, \hspace{3pt} \tau(1) = q_f, \hspace{3pt} \dot{q}_s = \dot{q}_f = 0$
\end{center}
where $q_s, q_f \in \mathcal{R}$ correspond to the static start and end joint configurations of the robot.
\end{definition}


==> definitions/control-projection.tex <==
\begin{definition}[Control Projection Function]\label{def:projection}
The \textsl{control projection function} $proj_{MP}$ projects a robot kinodynamic rollout $e \in \mathcal{K}_{MP}$ to a weighted, primitive--specific kinodynamic rollout, i.e.,

\begin{center}
$e^* = proj_{MP}(e)$
\end{center}

where $e^* \in \mathcal{M}_{MP}$.
\end{definition}


==> definitions/forward-model.tex <==
\begin{definition}[Forward Model]\label{def:forward-model}

Given an initial configuration $x_k \in \mathcal{X}$ and a set of feasible control parameters $u \in \mathcal{U}_{MP}$, the \textsl{forward model} $f_{MP}$ for a motion primitive $MP$ returns the final configuration $x_{k+1} \in \mathcal{X}$, i.e.,

\begin{center}
$x_{k+1} = f_{MP}(x_k, u)$
\end{center}
\end{definition}

where $\mathcal{U}_{MP}$ is the set of feasible control parameters for the chosen motion primitive $MP$.


==> definitions/situated-kinodynamic-manifold.tex <==
\begin{definition}[Situated Kinodynamic Manifold]\label{def:situated-manifold}
A \textsl{situated kinodynamic manifold} is a primitive--specific kinodynamic manifold, grounded in environmental configuration via a projection function $proj_{MP}$
\begin{center}
$\mathcal{M}_{MP} = \{(\mathcal{K}_{MP}, \rho) \mid proj_{MP}(e) \in \mathbb{R}\}$
\end{center}
where $e \in \mathcal{K}_{MP}$.
\end{definition}

==> evaluation-planner-new.tex <==
\subsection{Planner Evaluation}\label{sec:planner_eval}
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/planner_eval_smol.pdf}
%     \caption{Representative Scenario Solutions. Each image represents how the robot solved the scenario for each failure case. The colored lines are the motions of the robot end effector tip, with the color representing the manipulability of the robot. For each, the yellow boxes represent the target object or objects. The black outlined boxes in the first scenario represent the obstacles. For the first two scenarios, the black lines represent the motion of the target object. For visual simplicity, the final scenario only shows the final positions of the target objects.}
%     \label{fig:planner_ops}\vspace{-15pt}
% \end{figure*}



\subsubsection{Behavior of the Planner} 
We analyze the planner's quality through its behavior in the two failure scenarios through an analysis of the robot's actions to complete the tasks. For some of the cases, we will discuss two examples, one good and one bad, to understand better how the planner can be limited. In each of the cases, in \cref{fig:planner_ops}, we see the path the target object or objects took, the final position of any obstacles, and the path of the robot's end effector tip colored by the manipulability of the arm through the path.

\textbf{Failure Case 1}: In Test Scenario 1, we see the error in the sim-to-real action execution. The planner commands several actions, but the actions executed on the robot fail to move the target object from its initial position. During that time, the robot rearranges the obstacle objects significantly. Once the robot moves the target object initially, the arm is then able to execute a strong action and move the target object deep into the goal region.

In Test Scenario 2, we see the robot initially staying clear of the tunnel and then poking its end effector under the tunnel to move the object into the goal region outside of its reachable range.

Test Scenario 3 highlighted the challenges of manipulating objects near the edge of the robot's working space. Many of the actions here didn't go smoothly and had low manipulability throughout, causing significant discrepancies between what the simulation predicted and what the real robot could achieve. As a result, it took a total of eleven actions to move all four objects to the target region successfully.

\textbf{Failure Case 2}: In Test Scenario 1, we see that the scenario was completed in two actions, with each action moving the block in the direction of the goal. This represents the best-case scenario of the planner, where the sim-to-real system has very small errors and will move the object consistently with the goal of shrinking the gap to the target area. 

In Test Scenario 2,  we see how errors in the sim-to-real system can lower the performance of the planner. For this scenario, the planner commanded the robot to execute six actions. In the simulation-in-the-loop, these six actions interact with the target object and move it towards the goal. However, we only see the target object move five steps from the initial position to the goal; thus, the robot misses touching the target object entirely. There was only minimal contact between the arm and the object for two of the actions, causing only small movements. 

In Test Scenario 3, the robot efficiently moves three of the four target objects to the goal region with just two actions. However, those first two motions knock the fourth object away from the robot to an area with consistently lower manipulability. This means the planner commands four actions before a quality contact is made and the target reaches the goal.
\subsubsection{Strengths}
% greedy approach can lead to quick solutions and does not require optimization tuning 
% multi object manipulation
% dynamic interaction point -- no concern about which point on the robot an object touches, means the planner can make both sweeping actions across multiple object simultaneously and delicately control a single object
One of the key advantages of the planner is its efficient nature, thanks to a greedy approach that prioritizes quick solutions without the need for extensive optimization tuning. This quality expedites the planning process and simplifies the implementation of complex tasks. Furthermore, the planner excels in multi-object manipulation scenarios, where it can seamlessly coordinate the robot arm's movements to interact with multiple objects simultaneously. Its ability to manage dynamic interaction areas, irrespective of which part of the robot touches an object, allows for sweeping actions across multiple objects and delicate, precise control when dealing with a single object. This flexibility and adaptability make the task and motion planner a valuable tool for a wide range of robotic applications, where speed, versatility, and precision are paramount.

\subsubsection{Weaknesses}
% Greedy approach can lead to suboptimal actions and long plans
% scoring method for edge selection is too simple, can not remember what makes a 'good' action so repeatability is bad
% Sim to real can be very wrong
% sim in loop can increase planning times
% imperfect dynamics model for edge generation leads to even more error between simulation actions and real actions
One notable limitation is the use of a greedy approach, which, in certain scenarios, may result in suboptimal actions and lead to longer less efficient plans. Additionally, the planner relies on a relatively simple scoring method for edge selection, which lacks the ability to remember what constitutes a `good' action, resulting in poor repeatability. The challenge of sim-to-real transition can also pose difficulties, as the planner may struggle to accurately replicate real-world actions from simulations, leading to discrepancies and errors. Moreover, incorporating simulation-in-loop can increase planning times, potentially affecting real-time applications negatively. Lastly, the imperfect dynamics model used for edge generation can further exacerbate the gap between simulated actions and real-world outcomes. Despite these weaknesses, the planner's advantages make it a valuable tool for various robotic tasks when used judiciously and with consideration of these limitations.

These experiments show that \textbf{our approach successfully utilizes the kinodynamic map and the increased reachability of the robot arm to complete manipulation tasks in the face of LMJ through the use of non-prehensile movements, supporting H.2.}



==> evaluation-planner.tex <==
\subsection{Planner Evaluation}\label{sec:planner_eval}
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/success_rate_r_c.png}
         \caption{Success Rate}
         \label{fig:succ_rate}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/stacked_bar_c.png}
         \caption{Planning Time and Execution Time}
         \label{fig:exec_rate}
     \end{subfigure}
    \caption{Success rate, planning time, and execution time across different scenarios and failures\vspace{-10pt}}
    \label{fig:experiments}
\end{figure}
In many locked-joint failure combinations, the end-effector would be in a configuration that would severely limit its ability to grasp. However, in this work we want to eliminate the need for restrictions on the robot's kinematic configurations prior to failure to maximize the utility of the robot. With these two conflicting constraints, we must move beyond the exclusive use of end effectors to complete tasks. Furthermore, the increased area with which the robot can interact with the surrounding environment increases the efficacy of manipulating clutter, with actions often moving multiple objects at a time. In these results, summarized in \cref{fig:succ_rate,fig:exec_rate}, we show that our approach of leveraging whole-arm contact combined with multimodal actions allows the robot to complete tasks that would not be possible with grasp only approaches.

\subsubsection{Experiments with Failure Case 1} Our approach allows the robot to operate where grasp-only methods would fail completely, as seen in \cref{fig:reach_comp}. The findings of Failure Case 1 show that this case significantly hampers the abilities of the robot. In Scenario 1 the success rate was 20\%; the success was severely hampered by the interactions from the moveable obstacles pushing the target object outside of the limited reachable area, however, it is still a success given that the robot was unable to move its end effector to the goal region. Scenario 2 fared much better, with a 75\% success rate and a much improved task time over Failure Case 1, given that the system was able to utilize actions across the wrist and end-effector to interact with the objects.

\subsubsection{Experiments with Failure Case 2} The experimental findings garnered from Failure Case 2 attest to the capacity of the system to undertake demanding tasks that necessitate the robot to maneuver objects beyond its accessible range. Since this failure case renders the end-effector unusable, prior work \cite{brooks2016analysis} would not be applicable in addressing this Failure Case. The lower task times of this failure case in Scenario 1 was aided by the ability to interact with multiple objects at once. Across scenarios, the system worked consistently in managing the failure case, as seen in \cref{fig:succ_rate}, with 90\% success rate in Scenario 1 and 80\% success in Scenario 2. The outcomes provide compelling evidence of making full use of the available embodiment through non-prehensile actions and whole arm manipulation.

\subsubsection{Planning and Execution Times} Across the failure case and scenario combinations, the execution times for completing the tasks ranged between an average of 6 and 35 seconds, as highlighted in \cref{fig:exec_rate}. This demonstrates that, even when hindered by rapid-onset failures, the system was able to utilize the increased range and whole-body interaction to quickly complete these tasks. The planning times were a significant portion of the overall task time, also shown in the timeline of \cref{fig:timeline}. This can be attributed to our use of sim-in-the-loop edge selections, as shown in \cref{algo:adaptr}. However, as will be discussed in \cref{sec:conclusion}, future work can lower this overhead significantly.

The results show that \textbf{taking advantage of the whole embodiment of the robot, combined with non-prehensile actions, facilitates the robot's ability to accomplish tasks in the face of debilitating failure states. In other words, without \textit{ADAPT-R}, the robot would be unable to complete the tasks at hand, proving H.2.}

==> methods-edge-bundles.tex <==
\subsection{Situated Kinodynamic Manifold}\label{sec:edge-bundles}

Given the highly varied nature of prehensile and nonprehensile motion primitives, it may not always be possible to simulate multiple control parameters for each motion primitive within a reasonable amount of time. Moreover, doing this repeatedly for new planning problems with no memory of past experience adds to the computational cost of planning kinodynamically--feasible paths in high--dimensional workspaces.

Our work extends the concept of kinodynamic edge bundles to the multimodal domain by sampling edges based on forward simulation of the robot dynamics model \cite{shome2021asymptotically}. We term this \textsl{kinodynamic manifold} since it represents a generic set of primitive--agnostic edges that leads us to the definition of a \textsl{situated kinodynamic manifold}. More specifically, a \textsl{kinodynamic manifold} is a set of valid rollouts of the manipulator dynamics model generated by applying randomly sampled joint velocities at random joint configurations for a sampled period of time, thereby connecting random start configurations to resultant end configurations:
\begin{center}
% \begin{align}
$\mathcal{K}_{MP} = \{(x_s, x_f, u, \Delta t) \mid x_f = f_{MP}(x_s, u, \Delta t)\}$
% \end{align}
\end{center}
where $x_s, x_f \in \mathcal{X}$, $u \in \mathcal{U}_{MP}$, and $\Delta t \in \mathbb{R}$.
% such that $f_{MP}(x_s, u, \Delta t) = x_f$.
% where $|\mathcal{E}_{MP}| = m$.


% \input{definitions/kinodynamic-manifold.tex}

The manipulator dynamics model (\Cref{algo:generate-kinodynamic-manifold}, L12) is defined (here, for a 7DoF robot arm) as 
\begin{center}
$\tau = M(q)\ddot{q} + C(q, \dot{q})\dot{q} + g(q) + f(\dot{q})$
\end{center}
\begin{align*}
q_{min} &\leq q \leq q_{max}\\
-\dot{q}_{max} &\leq \dot{q} \leq \dot{q}_{max}\\
-\tau_{max} &\leq \tau \leq \tau_{max}\\
\end{align*}
where $q$ is a $7\times1$ vector representing the robot joint angles, $\dot{q}$ is the joint velocity $7\times1$ vector, $\tau$ is the $7\times1$ vector defining joint torques, $M$ is a positive-definite, symmetric $7\times7$ joint inertia matrix, $C$ is a $7\times7$ matrix that represents the Coriolis and centrifugal effects of robot motion, $g$ is a $7\times1$ vector that describes the amount of torque each motor needs to apply to oppose gravity, and $f$ is a $7\times1$ vector that denotes the torques needed to overcome joint friction.

To generate the \textsl{kinodynamic manifold}, a valid end--effector pose is sampled denoting the start configuration of the robot. Random end--effector velocity and duration is also sampled (\Cref{algo:generate-kinodynamic-manifold}, L3-6). These initial states are unrolled forward in time using the manipulator dynamics model while checking for joint position, velocity, acceleration, and torque limits, in addition to workspace limits and collisions with environmental objects (\Cref{algo:generate-kinodynamic-manifold}, L10-14). We additionally introduce a manipulability threshold and nullspace joint velocity sampling to ensure the rollout does not run into singularities or joint velocity limits (\Cref{algo:generate-kinodynamic-manifold}, L17).

% \input{definitions/control-projection.tex}

Adapting this robot kinodynamic manifold to specific motion primitives requires the introduction of a projection function $\mathcal{proj_{MP}}$ (\Cref{def:projection}). This function leverages a taxonomy of robot motions and environmental characteristics consisting of four interactions:
\begin{itemize}
\item robot only: This considers features of the robot kinodynamic manifold $\mathcal{K}_{MP}$ such as manipulability, dynamic manipulability, and reachability and assigns a weighting on on their quantitative measurements.
\item robot--object: This type of interaction considers the compatibility of robot and object characteristics such as relative gripper--object size and how object height dictates end--effector positioning for nonprehensile manipulation.
\item robot--environment: Here, we ensure that the robot does not collide with movable or fixed obstacles unintentionally. Distribution of clutter and ensuring $e \in \mathcal{K}_{MP}$ has sufficient clearance to execute successfully also informs this metric.
\item object--environment: For nonprehensile interactions, the Coulomb friction between the object and its support surface determines the success of an action. For instance, it is more beneficial for poking to operate in low friction environments to take maximal advantage of its capacity to extend the robot's reachable space. However, the threshold is higher for pushing since constant contact between the robot and the object ensures continuous object motion.
\end{itemize}

Combined, these interactions allow us to quantify the effectiveness of $e \in \mathcal{K}_{MP}$ for a given primitive and operational scenario via $proj_{MP}$, further allowing us to create a \textsl{situated kinodynamic map} for each primitive, grounded in object characteristics and environment configuration.
\ap{more?, see utility.py, task based?, talk about culling edges for poking and grasp action sampling (in planner?)}

% i) robot only, ii) robot--object, iii) robot--environment, iv) object--environment, and, v) task--based.
% \ap{talk about it here, adapt skill + utility, talk about contact taxonomy, what features for each skill, scene--dep weighting}

% \input{definitions/situated-kinodynamic-manifold.tex}

% \subsubsection{Real--World Considerations}
% \ap{talk about ramp up and ramp down}



==> methods-formalization.tex <==
\subsection{Formalization of Motion Primitives}\label{sec:motion-primitives}

As motivated in \Cref{sec:introduction}, there exist a variety of prehensile and nonprehensile motion primitives, each with its core set of capabilities and limitations.
We unify this diverse portfolio under a single definition of \textsl{motion primitive} $MP$ as an entity with four components: 
i) $f_{MP}$, a forward model (\Cref{def:forward-model}); 
ii) $\phi_{MP}$, a control mechanism for generating the robot--object motion (\Cref{def:control-mechanism}); 
iii) $\mathcal{M}_{MP}$, a situated kinodynamic manifold (\Cref{def:situated-manifold}); and, 
iv) $proj_{MP}$, a control projection function (\Cref{def:projection}).
A more extensive treatment of these components and our design choices is presented in the context of our motion planning framework in \Cref{sec:methods-planning}. 

% \begin{enumerate}
%     \item $f_{MP}$, a forward model that computes the final object pose from an initial pose and a set of control parameters (\Cref{def:forward-model});
%     \item $\phi_{MP}$, a control mechanism for generating the robot--object motion resulting from a set of control parameters (\Cref{def:control-mechanism});
%     \item $\mathcal{M}_{MP}$, a situated kinodynamic manifold that maps the current environment state and primitive control parameters to a real value to determine goodness of action (\Cref{def:situated-manifold}); and,
%     \item $proj_{MP}$, a control projection function that maps a generic robot dynamics rollout to the primitive's situated kinodynamic manifold, thus allowing for experience reuse (\Cref{def:projection}).
% \end{enumerate}

% \input{definitions/forward-model.tex}
% \input{definitions/control-mechanism.tex}

In this work, we leverage \textsl{poking} as our motion primitives for \gm{give a reason}. A discussion of its characteristics is provided next.

==> methods-selection.tex <==
\subsection{Selection of Motion Primitive}\label{sec:methods-selection}

As motivated in \Cref{sec:introduction}, robot capability, object characteristics, and environment configuration inform the need for a diverse repertoire of prehensile and nonprehensile motion primitives.
In this section, we provide a functional definition of our chosen primitive of \textsl{poking}.

\textsl{Poking} is a fundamental nonprehensile motion primitive that is composed of two sequential phases: i) \textsl{impact}: a robot end-effector applies an instantaneous force to an object at rest, setting it in planar translational and rotational motion; and, ii) \textsl{free-sliding}: the object slows down and comes to a halt due to Coulomb friction between the object and its support surface \cite{pasricha2022pokerrt}. This primitive is not limited by robot reach and leads to faster manipulation of objects. However, poking is limited by robot dynamics and nonlinearities due to friction between the object and its support surface \ap{cite}.



==> related.tex <==

Locked joint failures have been studied in  \cite{mu2016kinematic}, \cite{xie2021maximizing}, and \cite{lewis1997fault}. Zonggao et al. \cite{mu2016kinematic} worked on kinematic analysis and fault-tolerant trajectory planning of a non-redundant spatial manipulator under single joint failure. They calculated inverse kinematics using an analytical method. Then they combined it with the desired end-effector performance and employed the concept of fault tolerance angle for trajectory planning under failure. Xie et al. \cite{xie2021maximizing} presents an algorithm to compute the trajectory with the maximum probability of completing a set of point to-point tasks after a locked joint failure. It finds shortest distances between the self-motion manifold joint regions of a point-to-point task. Lewis et al. \cite{lewis1997fault} presented a method to ensure a manipulator can still complete a task even after a locked joint failure. It involves analyzing self-motion manifolds and imposing joint constraints to guarantee reachability. The approach allows for entire regions of the workspace to be reachable even after any joint failure. 

In \cite{banerjee2020tale}, \cite{mcguire2019everybody}, \cite{chang2013robot}, and \cite{brooks2016analysis} failure recovery is accommodated by a human operator. Banerjee et al. \cite{banerjee2020tale} focused on ways of providing decision support to human operators to help robots with failure recovery. The findings indicate that operators should receive both diagnosis and action recommendations for optimal effectiveness in failure recovery. McGuire et al. \cite{mcguire2019everybody} developed an adaptive approach to address failure recovery using a reinforcement learning method. In this approach, when a robot encounters a faulty state, it selects a human assistant to help in recovering from the fault. Chang et al. \cite{chang2013robot} suggest an automatic error recovery approach utilizing Petri nets. This approach enables the robot to recover from known errors and learn how to recover from unknown errors by observing a human demonstrator. Brooks et al. \cite{brooks2016analysis} conducted a survey experiment, they discovered that the perceived effectiveness of recovery strategies, as evaluated by humans, is impacted by the type and severity of the failure as well as the context in which it occurs. 

Du et al. \cite{du2017fault} presented a motion planning technique that enables a six-legged robot to cope with multiple broken legs using null space and Jacobian matrices.

Vonásek et al. \cite{vonasek2015online} proposed a system that employs a high-level motion planner which is equipped with a series of motion primitives, generated by locomotion generators. When a failure happens, the motion planner determines whether to use the existing motion primitives to execute a new plan or to adapt them using particle swarm optimization as necessary.  

Jamshidi et al. \cite{jamshidi2019machine} used Machine Learning to enable run-time self-adaptations and integration of information from multiple heterogeneous models in quantitative planning. Their focus is not on faulty joins but rather on quantitative constraints such as battery power.
\ava{todo for myself: connect to methods}

% One study by Lewis and Maciejewski \cite{r2} proposed a fault-tolerant operation method for kinematically redundant manipulators by identifying areas of the robot's workspace that guarantee failure recoverability using self-motion manifolds. They restricted the joints to certain ranges that maximize the local kinematic failure tolerance measure, which keeps the robot in configurations with large self-motion manifolds. Another study by Patarinsky-Robson et al. \cite{r3} presented an analytical method of recovering from locked joint failure of a 6-degree-of-freedom (dof) robot for failure in three different joints. The approach allowed the 6dof arm to complete a positioning task at any orientation.

% Du and Gao \cite{r5} proposed a method for tolerating multiple faults in a six-legged robot by using null space motion through Jacobian-based motion planning. The study showed that the robot can still locomote with several legs broken. Mu et al. \cite{r6} presented a kinematic analysis and fault-tolerant trajectory planning method for a non-redundant spatial manipulator under a single joint failure using an analytical method for inverse kinematics and maximizing the ability of the space manipulator under a single joint failure.

% Banerjee et al. \cite{r1} investigated the best ways to present a human operator with information about a robot's failure to provide recovery instructions. They presented an experiment in which participants were provided with suggestions for action recommendations and feedback on fault diagnosis. The results suggested that feedforward information (i.e., suggesting action recommendations) was the most useful to humans, and feedback (fault diagnosis suggestions) could supplement that information.

% Finally, McGuire et al. \cite{r7} proposed a reinforcement learning method for a robot to select a human assistant to aid in recovering from a fault. The method utilized a task analysis and monitoring to determine which human assistant would be best suited for the given task.

% In summary, the reviewed studies have proposed different approaches to handle various types of robot failures, including fault-tolerant operation, null space motion planning, and fault-tolerant trajectory planning. They have also investigated how to provide human operators with suggestions for recovery instructions and how to utilize human assistance to aid in fault recovery.


Jacobian projection--based constrained motion planning techniques face similar issues, in addition to failing to generalize to dynamic constraints \ap{cite}, which is the core for most nonprehensile motion primitives.
